Variational Information Maximisation for Intrinsically Motivated Reinforcement Learning

The mutual information is a core statistical quantity that has applications in all areas of machine learning, whether this is in training of density models over multiple data modalities, in maximising the efficiency of noisy transmission channels, or when learning behaviour policies for exploration by artificial agents. Most learning algorithms that involve optimisation of the mutual information rely on the Blahut-Arimoto algorithm --- an enumerative algorithm with exponential complexity that is not suitable for modern machine learning applications. This paper provides a new approach for scalable optimisation of the mutual information by merging techniques from variational inference and deep learning. We develop our approach by focusing on the problem of intrinsically-motivated learning, where the mutual information forms the definition of a well-known internal drive known as empowerment. Using a variational lower bound on the mutual information, combined with convolutional networks for handling visual input streams, we develop a stochastic optimisation algorithm that allows for scalable information maximisation and empowerment-based reasoning directly from pixels to actions.

==> conclusion.tex <==
\section{Discussion and Conclusion}

==> internal_notes.tex <==
\section{Scalable Mutual Information Optimization}

We can optimize the MI bound without the use of a model and our optimizer can be fully integrated within a standard RL framework.

First note that maximizing the MI wrt the policy is in general an ill-posed problem (e.g. linear models, where the policy's covariance matrix diverges).

Therefore we maximize the MI under the constraint that the entropy of the policy is bounded by adding a constraint.

The variational bound and entropy constraint are combined below
\begin{align}
\mathcal{J}^{\pi}(s) &= \E_{ p(s' | s, A) \pi(A|s) } [ - \frac{1}{\beta} \ln \pi(A|s) + \ln q(A|s,s') ] \nonumber\\
&=\E_{ p(s' | s, A) \pi(A|s) } [ \Lambda(s,A,s') ], \label{eq:objective}
\end{align}
where $A$ is the history of actions performed by the agent when moving from $s$ to $s'$ and $\beta$ is an inverse-temperature.

Here $\mathcal{J}^{\pi}(s)$ plays the role of a value-function and $\Lambda(s,A,s')$ plays the role of a $Q$-function.

The quantity $\mathcal{J}^{\pi}(s)$ is to be optimized with respect to both $\pi(A|s)$ and $q(A|s,s')$.

Optimization with respect to $q(A|s,s')$ is a simple supervised maximum-likelihood problem.

We note that the optimal policy ( computed by solving $ \delta \mathcal{J}^{\pi}(s) / \delta \pi(A|s) = 0 $ under the constraint that $\sum_{A} \pi(A|s) = 1$   ) is given by

\begin{align}
\pi(A|s) &= \frac{1}{Z(s)} e^{ \beta \E_{p(s' | s, A)}[ \ln q(A|s,s') ]  }, \nonumber \\
&= \frac{1}{Z(s)} e^{ \beta \phi(s,A)  } \label{eq:optimal_policy}
\end{align}
where $Z(s) = \sum_{A} e^{ \beta \phi(s,A)  } $ is a normalization term and $\phi(s,A) = \E_{p(s' | s, A)}[ \ln q(A|s,s') ] $ .

If we replace the optimal policy \eqref{eq:optimal_policy} in the objective function \eqref{eq:objective} we can write it in terms of the normalization function only:

\begin{align}
\mathcal{J}^{\star}(s) &= \frac{\ln Z(s)}{\beta}.
\end{align}

\subsection{Two-point algorithm}

The optimal policy is only implicitly defined by \eqref{eq:optimal_policy} and there is no direct mechanism for sampling actions or computing the normalizing function $Z(s)$. We could, for instance, use a simple importance sampling approximation. But this solution is not satisfactory as it required several evaluations of $\phi(s,A)$ per decision.

We propose a (new?) method for approximating unnormalized distributions by a normalized parametric distribution below.


Given an unnormalized density $ p(x) \propto e^ {\phi(x)} $ we introduce the normalization-independent function $f_p(x,x')$ 
\begin{align}
f_p(x,x') &= \phi(x) - \phi(x'),
\end{align}

Note that the function $f_p(x,x')=-f_p(x',x)$ entirely characterizes the density $p(x)$ which can be written as 

\begin{align}
p(x) &= \left[  \int dx' e^{f_p(x',x)}  \right]^{-1}.
\end{align}

In order to approximate $p(x)$ by a normalized parametric density $q(x)$ we minimize with respect to $q(x)$  the loss function:

\begin{align}
C[q] &= \int dx dx' \rho(x,x') || f_p(x,x') - f_q(x,x') ||^2,
\end{align}

where $\rho(x,x')$ is any density with same support as $p(x)$.

\subsubsection{Proof of convergence for discrete distributions}


Let $x\in N^d$ be a discrete domain and $p(x)$ be a probability vector.

\begin{align}
C[q] &= \sum_{x,x'}  || \ln  q(x) - \ln  q(x') - \ln  p(x) + \ln  p(x') ||^2/4 - \lambda \sum_x q(x),
\end{align}


\begin{align}
\frac{dC[q]}{dq(x)} &= \sum_x \left [\ln  q(x') - \ln  q(x) - \ln  p(x') + \ln  p(x) \right] -\lambda q(x) \nonumber \\
&=0 \\
\ln q(x') &= \sum_x \ln q(x) + \ln p(x') - \sum_x \ln p(x) + \lambda q(x) \\
\end{align}



\subsection{random comments}

- predictability?  

==> intro.tex <==
\section{Introduction}
\vspace{-2mm}
%The applicability of machine learning systems continues to expand at a rapid rate, and now forms the core of an extremely diverse set of applications. In image classification, we now have systems that allow highly accurate class assignments without hand-designed features [], in reinforcement learning, we have highly accurate systems that can learn behaviour policies from high-dimensional sensory streams \citep{mnih2013atari}, and in text analysis, we now routinely extract topics and categories from large volumes of legal and scientific documents. These systems have made advances by expanding upon well established problems such as learning discriminative functions or density models, and then developing inference methods that at the outset have low computational complexity, that use unified loss functions that make it easier to reason about the problem, and stochastic optimisation to allow for large-scale learning. 

The problem of measuring and harnessing dependence between random variables is an inescapable statistical problem that forms the basis of a large number of applications in machine learning, including rate distortion theory \citep{coverThomasInfo}, information bottleneck methods \citep{tishby2000information}, population coding \citep{agakov2004algorithm}, curiosity-driven exploration \citep{still2012information, rubin2012trading}, model selection \citep{infoTheoryModeSelect}, and intrinsically-motivated reinforcement learning \citep{empowermentIM}. In all these problems the core quantity that must be reasoned about is the mutual information. 
%While many other areas of machine learning, such as image classification, reinforcement learning and text analysis have seen rapid advances and applicability at scale, information maximisation problems -- problems involving optimisation of the mutual information -- have lagged. %It is this gap that we address. 
In general, the mutual information (MI) is intractable to compute and few existing algorithms are useful for realistic applications. The received algorithm for estimating mutual information is the  Blahut-Arimoto algorithm \citep{YeungBA2008} that effectively solves for the MI by enumeration --- an approach with exponential complexity that is not suitable for modern machine learning applications.  
%What other currently successful areas of machine learning have in common is that they exploit inference methods that at the outset were designed with low computational complexity, that use unified loss functions that make it easier to reason about the problem, and that use stochastic optimisation to allow for large-scale learning.  
By combining the best current practice from variational inference with that of deep learning, we bring the generality and scalability seen in other problem domains to information maximisation problems. We provide a new approach for maximisation of the mutual information that has significantly lower complexity, allows for computation with high-dimensional sensory inputs, and that allows us to exploit modern computational resources. 

The technique we derive is generally applicable, but we shall describe and develop our approach by focussing on one popular and increasingly topical application of the mutual information: as a measure of `empowerment' in intrinsically-motivated reinforcement learning. Reinforcement learning (RL) has seen a number of successes in recent years that has now established it as a practical, scalable solution for realistic agent-based planning and decision making \citep{mnih2013atari, koutnik2014evolving}. A limitation of the standard RL approach is that an agent is only able to learn using external rewards obtained from its environment; truly autonomous agents will often exist in environments that lack such external rewards or in environments where rewards are sparsely distributed. \textit{Intrinsically-motivated reinforcement learning} \citep{singh2005intrinsically} attempts to address this shortcoming by equipping an agent with a number of internal drives or intrinsic reward signals, such as hunger, boredom or curiosity that allows the agent to continue to explore, learn and act meaningfully in a reward-sparse world. There are many ways in which to formally define internal drives, but what all such definitions have in common is that they, in some unsupervised fashion, allow an agent to reason about the value of information in the action-observation sequences it experiences. 
The mutual information allows for exactly this type of reasoning and forms the basis of one popular intrinsic reward measure, known as \textit{empowerment}.
%For realistic agent-based systems, we require that any measure of internal reward be independent of any specific task, be easily computable or amenable to efficient approximation, and be easily composed with existing reinforcement learning methods. And one of promising and popular intrinsic reward is known as \textit{empowerment} whose definition is based on the mutual information.

Our paper begins by describing the framework we use for online and self-motivated learning (section \ref{sect:imrl}) and then describes the general problem associated with mutual information estimation and empowerment (section \ref{sect:empowerment}). We then make the following contributions:
\vspace{-3mm}
\begin{itemize}[leftmargin=*]
\setlength{\itemsep}{0pt}
\setlength{\parskip}{0pt}
\setlength{\parsep}{0pt}
\item We develop \textit{stochastic variational information maximisation}, a new algorithm for scalable estimation of the mutual information and channel capacity that is applicable to both discrete and continuous settings.
\item We combine variational information optimisation and tools from deep learning to develop a \textit{scalable algorithm for intrinsically-motivated reinforcement learning}, demonstrating a new application of the variational theory for problems in reinforcement learning and decision making.
\item  We demonstrate that empowerment-based behaviours obtained using variational information maximisation match those using the exact computation. We then apply our algorithms to a broad range of high-dimensional problems for which it is not possible to compute the exact solution, but for which we are able to act according to empowerment --  \textit{learning directly from pixel information}.
\end{itemize}


%
%Reinforcement learning (RL) has seen a number of successes in recent years that has now established it as a practical, scalable solution for realistic agent-based planning and decision making. These successes include playing Atari games with super-human performance \citep{mnih2013atari, guo2014deep}, learning controllers for 3D racing simulators \citep{koutnik2014evolving}, or leaning to play the game of Go \citep{clarkConvGo2014}. What these approaches have in common is that they exploit the power of \textit{deep reinforcement learning}, which uses deep neural networks as powerful non-linear function approximators for value estimation, allowing for agents that can now learn directly from pixels to actions.
%% At the same time, \textit{variational inference} has emerged as the corresponding approach for tractable and scalable probabilistic inference, based on introducing lower bounds on difficult to compute probabilistic quantities.
%A limitation of the standard RL approach is that the agent is only able to learn using external rewards obtained from the environment; truly autonomous agents will often exist in environments that lack such external rewards or in environments where rewards are sparsely distributed. \textit{Self-motivated reinforcement learning} attempts to address this shortcoming by equipping an agent with a number of internal drives or intrinsic reward signals, such as hunger, boredom or curiosity that allows the agent to continue to explore, learn and act meaningfully in a reward-sparse world. 
%In this paper, we  combine the successes  of deep reinforcement learning with principled and tractable objective functions obtained using variational inference to develop a new scalable approach for intrinsically-motivated reinforcement learning. 
%%using insights and successes from deep reinforcement learning and a variational approximation for an information-theoretic intrinsic reward, to develop the first scalable approach for intrinsically-motivated RL. 
%
%There are many ways in which to formally define internal drives, but what all such definitions have in common 
%%While there are a number of approaches for specifying internal drives that have been proposed, what they have in common 
%is that they, in some unsupervised fashion, allow the agent to reason about the value of information in the action-observation sequences it experiences. %it perceives. 
%For realistic agent-based systems, we require that any measure of internal reward be independent of any specific task, be easily computable or amenable to efficient approximation, and be easily composed with existing reinforcement learning methods. We choose an information-theoretic measure that meets these requirements known as \textit{empowerment} %\citep{klyubin2005empowerment} % 
%~\citep{salge2014empowerment}. 
%Empowerment is a measure of the channel capacity or maximum mutual information between a sequence of actions and the final state reached by executing those actions. This makes empowerment a compelling self-motivation-measure, since by using empowerment an agent is able to quantify its degree of control over an environment from any starting state, i.e. its ability to reach any future state in many ways. We shall demonstrate that this knowledge leads an `empowered' agent to exhibit interesting and useful behaviours.
%
%Since the mutual information is central to the definition of empowerment, its efficient estimation is the focus of this paper. In general, the mutual information is intractable to compute and few existing algorithms are useful for realistic applications of the mutual information, whether for rate distortion theory \citep{coverThomasInfo}, population coding \citep{agakov2004algorithm}, information-bottleneck methods \citep{tishby2000information}, reinforcement learning \citep{still2012information, rubin2012trading}, or empowerment.
%
%Our paper begins by describing our general framework for intrinsically motivated reinforcement learning (section \ref{sect:imrl}) and the definition and intuition for empowerment (section \ref{sect:empowerment}). We then make the following contributions:
%\vspace{-3mm}
%\begin{itemize}[leftmargin=*]
%\setlength{\itemsep}{0pt}
%\setlength{\parskip}{0pt}
%\setlength{\parsep}{0pt}
%\item We develop stochastic variational information maximisation, a new algorithm for scalable estimation of the mutual information and channel capacity that is applicable to both discrete and continuous settings.
%\item We focus on empowerment as one well motivated drive for acting in the absence of external rewards. We combine variational information optimisation and recent advances in deep learning to develop a scalable method for intrinsically motivated reinforcement learning, demonstrating a new application of the variational theory for problems in reinforcement learning and decision making.
%\item We demonstrate that empowerment-based behaviours obtained using variational information maximisation match those using the exact computation. We then apply our algorithms to a broad range of high-dimensional problems for which it is not possible to compute the exact solution, but for which we are able to act according to empowerment --  learning directly from pixel information.
%\end{itemize}
%
%%
%% Old intro
%% Progress in machine learning towards developing autonomous systems and agents has for the most part focussed on agents that learn and act based on external guidance, whether this be in supervised learning and classification of complex image scenes \citep{szegedy2014going}, or external reward signals in reinforcement learning \citep{mnih2013atari}.  While these are essential components of any and intelligent system, truly autonomous agents will often exist in environments in which there are sparse or no external reward signals available. 
%%\dcom{ Not very happy with this first paragraph, but I don't have good suggestions for it yet }
%% Biological agents deal with this inevitability by employing a number of internal drives or intrinsic reward signals, such as hunger, boredom or curiosity that allows the agent to continue to explore, learn and act meaningfully in the world. It is with this problem in mind that we explore and develop a new scalable information-theoretic approach for problems in machine learning and intrinsically motivated reinforcement learning.
%%
%%We explore the intrinsic reward known as \textit{empowerment} \citep{klyubin2005empowerment, salge2014empowerment}. Empowerment is a measure of the channel capacity or maximum mutual information between a sequence of actions and the final state reached by executing those actions. This makes empowerment an extremely interesting measure, since by using empowerment an agent is able to quantify its degree of control over its environment from any starting state, i.e. its ability to reach any future state in many ways. In an empowered state, actions take by the agent will maximally influence the future states of the environment within its planning horizon.
%%%, an agent will have the maximum MI, indicating that the actions it can take from an empowered state gives the agent the maximal amount of information about future states. Reasoning in this way, the agent is able to act in environments in an unsupervised manner, without external reward. 
%% % % % % % %
%%The mutual information (MI) is a core statistical quantity and its efficient estimation is the focus of this paper.
%%The MI has several useful and intuitive interpretations and we shall often refer to the mutual information between a \textit{source} and its \textit{response}: in statistics, it is a multivariate measure of correlation between two random variables; in neuroscience the MI measures the efficiency of transmitting information between the input and output of neural circuitry; similarly, in communications theory the MI measures the efficiency of a noisy channel in transmitting information through the channel; in control theory the MI is used  a measure of the difference between a controlled and uncontrolled state of a system. 

==> otherBounds.tex <==
\section{Alternative Lower Bounds on the Mutual Information}
\label{sect:app_MIBounds}
In this section we briefly derive alternative lower bounds on the mutual information. Throughout we will consider the mutual information $\mathcal{I}(x,y)$ between a source $x$ and a response $y$.

\subsection{Variational Information Lower Bound}
The variational information lower bound \citep{agakov2004algorithm} introduces a variational distribution $q(x |y)$. Using the derivation from section \ref{sect:MI}, this bound is:
\begin{eqnarray}
\mathcal{I}(x,y) &=& H(x) - H(x|y) \\
 &\geq & H(x) - \expect{p(y|x)p(x)}{\log q_\xi (x | y)}\\
 & = & \mathcal{I}_{VI}
\end{eqnarray}
This bound is extremely convenient, since the distribution $p(y |x)$ can be interpreted as an encoder, with the distribution $q(x | y)$ as the corresponding decoder. This bound becomes exact when the varitaional distribution equal the true posterior distribution, i.e. when $q(x | y) = p(x | y)$.

\subsection{Fisher Bound}
The Fisher bound \citep{brunel1998mutual} rewrites the mutual information in the following form:
\begin{eqnarray}
\mathcal{I}(x,y) &=& \iint p(x,y) \log \frac{p(x,y)}{p(x)p(y)} dx dy \\
& = & \iint p(x,y) \log \frac{p(y|x)}{p(y)} dx dy \\
& = & \iint p(y|x)p(x)\log p(y|x) dx dy \nonumber \\
& & - \iint p(y,x) \log p(y) \\
& = & H(y) - \int p(x) H(y|x) dx
\end{eqnarray}
where $H(\cdot)$ is the entropy. We can now make the argument that the true distribution $p(y|x)$ can be estimated using a Gaussian distribution $\mathcal{N}(y | \hat{y}, \sigma_y^2)$, whose mean $\hat{y} = \expect{p(y |x)}{y}$ and a variance given by the inverse of the Fisher information $\sigma_y^2 = 1/\mathcal{J}(y)$; $\mathcal{J}(y) = \expect{p(y)}{\frac{\partial^2 \log p(x |y)}{\partial y^2}}$. We know then that the entropy term $H(y|x)$ for a Gaussian is only dependent on the variance and hence only on the inverse Fisher information. By appealing to the Cramer-Rao lower bound, we also know that no other estimator can have a variance lower than this, which allows us to obtain a bound on the entropy and hence the mutual information in terms if the mutual information.
\begin{eqnarray}
\mathcal{I}(x,y) & = & H(y) - \int p(x) H(y|x) dx \\
&\geq & H(y) - \int p(x) \frac{1}{2}\log \frac{2\pi e}{\mathcal{J}(y)} dx \\
& = & H(y) - \expect{p(x) }{\frac{1}{2}\log \frac{2\pi e}{\mathcal{J}(y)}}  dx \\
& = & \mathcal{I}_{Fisher}
\end{eqnarray}
In the asymptotic regime, this bound also becomes exact, but computation of the inverse Fisher information is a computationally expensive task and does not usually lead to scalable algorithms.

\subsection{Log Bound}
The log bound \citep{jaakkola1998improving} developed a bound on the mutual information in the mixture modelling setting using the convexity bound for the logarithm:
\begin{equation}
-\log x \geq - \lambda x + \log \lambda + 1
\end{equation}
This allows for a number of bounds to be developed and have been most widely used in local variational problems, though have been found to be too loose and alternative approaches are now preferred.


%begins by rewriting the mutual information as:
%\begin{eqnarray}
%\mathcal{I}(x,y) &=& \iint p(x,y) \log \frac{p(x,y)}{p(x)p(y)} dx dy \\
%& = & \iint p(x,y) \log \frac{p(y|x)}{p(y)} dx dy \\
%& = & \iint p(x,y) \left(-\log \frac{p(y)}{p(y|x)}\right) dx dy \\
%& = & \iint p(x,y) \left(-\log \frac{p(y)}{p(y|x)} \frac{q(y|x)p(x)}{q(y|x)p(x)}\right) dx dy \\
%& = & \iint p(x,y)\log q(y|x) -\int p(x)\log p(x) \nonumber \\
%& & + \iint p(x,y) \left(-\log \frac{p(y)q(y|x)}{p(x)p(y|x)}\right)
%\end{eqnarray}
%Were we have introduced a smoothing distribution $q(y|x)$. A bound can now be obtained by using the convexity bound for the logarithmic function:
%\begin{equation}
%-\log x \geq - \lambda x + \log \lambda + 1
%\end{equation}
%While bounds based on this approach have been applied in a number of local variational problems, alternative, tighter bounds are now preferred.
%%\section{Computing Mutual Information using a Generative Model} %
%%Maybe?



==> varAlg.tex <==
\section{Acting with Variational Empowerment}

\subsection{System Overview}

\subsection{Learning Models of the Environment}
\subsection{Computing Mutual Information}
\subsection{Empowerment-driven Policies}
\subsection{Computational Complexity}


